Involving External Stakeholders in Project Courses

Problem: The involvement of external stakeholders in capstone projects and project courses is desirable due to its potential positive effects on the students. Capstone projects particularly profit from the inclusion of an industrial partner to make the project relevant and help students acquire professional skills. In addition, an increasing push towards education that is aligned with industry and incorporates industrial partners can be observed. However, the involvement of external stakeholders in teaching moments can create friction and could, in the worst case, lead to frustration of all involved parties. Contribution: We developed a model that allows analysing the involvement of external stakeholders in university courses both in a retrospective fashion, to gain insights from past course instances, and in a constructive fashion, to plan the involvement of external stakeholders. Key Concepts: The conceptual model and the accompanying guideline guide the teachers in their analysis of stakeholder involvement. The model is comprised of several activities (define, execute, and evaluate the collaboration). The guideline provides questions that the teachers should answer for each of these activities. In the constructive use, the model allows teachers to define an action plan based on an analysis of potential stakeholders and the pedagogical objectives. In the retrospective use, the model allows teachers to identify issues that appeared during the project and their underlying causes. Drawing from ideas of the reflective practitioner, the model contains an emphasis on reflection and interpretation of the observations made by the teacher and other groups involved in the courses. Key Lessons: Applying the model retrospectively to a total of eight courses shows that it is possible to reveal hitherto implicit risks and assumptions and to gain a better insight into the interaction...

==> author-data-anon.tex <==
\acmformat{Anonymous. Involving External Stakeholders in Project Courses}

\begin{bottomstuff}

\end{bottomstuff}

\author{Anonymous}

\markboth{Anonymous}{Involving External Stakeholders in Project Courses}

==> model-application-summary.tex <==
\afterpage{
\begin{landscape}

\begin{table}[htbp]
\centering
\tbl{Application of the model to the different project courses, indicating both observations about the model as well as results from applying it. The table illustrates the different perspectives of the teachers and their different approaches to apply the model. The reflection only contains  weaknesses of the final iteration of the model since weaknesses in previous iterations were addressed.}{
 \begin{tabular}{@{}P{2cm}P{2.4cm}P{1cm}P{3cm}P{3.4cm}P{3cm}P{3cm}@{}}
 \toprule
 & & \multicolumn{3}{c}{\textbf{Observations}} & \multicolumn{2}{c}{\textbf{Results}} \tabularnewline
\textbf{Course} & \textbf{Stakeholders} & \textbf{Time needed} & \textbf{Strengths of model} & \textbf{Weaknesses of model} & \textbf{Lessons learned} & \textbf{Solutions} \tabularnewline
\midrule
CMPE450 & University employees as customers for the software that students are supposed to develop &  5 hours & Helpful in showing the peers current course design systematically \& clearly & Takes too long to complete the guide for model's sixth iteration \newline Requires time to grasp the big picture after filling in the model guide & A plan and feasibility analysis for the maintenance of the software that students developed must be made, if the software will be used in real life \newline Customers with no software engineering background may come up to the students with unrealistic requirements   & Discuss with university's IT staff  who are expected to take over software's maintenance before preparing the course project description. \newline Monitored the requirements gathering and elicitation process of students with customers and intervened when students got confused.\tabularnewline
\midrule
CMPE451 & Software practitioner and entrepreneur as course's primary teacher, and ICSE SCORE contest contact person &  4.5 hours (with some interruptions) & Model helps to think beforehand who the right candidates for external stakeholders are. \newline Shows the stakeholders that might have been implicitly introduced in the course without proper awareness.  & Template needs to be filled separately for each stakeholder with different roles and responsibilities &  External stakeholders whose engagement cannot be guaranteed should not be included to the course. \newline (In some cases) Teachers can prevent unpleasant consequences due to the lack of some external stakeholders' engagement by taking over their responsibilities.\tabularnewline
\midrule
CSC302 & Industrial guest lecturers, former lecturers, academic department & less than one hour & Explicit focus on the variety of stakeholders and their goals\newline Captured both known and previously unknown disconnects between important stakeholders & Aimed for the design of a new course, thus many redundant or not applicable questions for retrospective course analysis & External stakeholder use was misaligned to course content\newline More interestingly, the model brought to light issues with departmental support for guest lectures, and lack of governance & Instructor must coordinate with guest lecture, even if the contact is not theirs\newline  The department should provide more support and governance for the use of industrial lecturers, particularly for sessional instructors\tabularnewline
\midrule
DAT255/DIT543 & Product Owners, mentors, guest lecturers, jury & N/A & Questions mostly formulated for constructive use\newline Guideline has to be known in advance to avoid duplication & Identification of different types of stakeholders\newline Helped identify issues unrelated to stakeholder involvement & Little alignment of course objectives with program\newline No means to gauge whether aims of all involved parties are achieved\newline External stakeholders insufficiently prepared for their role\newline Teacher and stakeholder aims mismatched & Discussions on program level to improve cohesion\newline Clear statement of aims of all parties\newline Workshops and meetings with stakeholders to prepare them\tabularnewline
\bottomrule
\end{tabular}}
\label{tab:source-type-provenance-2}
\end{table}

\begin{table}[htbp]
\centering
\tbl{Application of the model to the different project courses, indicating both observations about the model as well as results from applying it. The table illustrates the different perspectives of the teachers and their different approaches to apply the model. The reflection only contains  weaknesses of the final iteration of the model since weaknesses in previous iterations were addressed.}{
 \begin{tabular}{@{}P{2cm}P{2.4cm}P{1cm}P{3cm}P{3.4cm}P{3cm}P{3cm}@{}}
 \toprule

& & \multicolumn{3}{c}{\textbf{Observations}} & \multicolumn{2}{c}{\textbf{Results}} \tabularnewline
\textbf{Course} & \textbf{Stakeholders} & \textbf{Time needed} & \textbf{Strengths of model} & \textbf{Weaknesses of model} & \textbf{Lessons learned} & \textbf{Solutions} \tabularnewline
\midrule
%\midrule

DAT265/DIT599 & Open source projects as product owners & (to apply the model) 1-2 hours & Easy to apply\newline Helped to document and cover aspects of the stakeholder interaction and set-up & Not all questions relevant for all courses (user needs to be selective hen filling in the guide) & Misalignment between treatment of newcomers in open source projects and the time frame of the course & Adapted assessment between two course instances to reduce the risk that students miss course goals by focussing too much on getting a contribution to the OSS project accepted \tabularnewline
\midrule
DIT029 & Industrial company & (to apply the model) 1-2 hours & Model helped identifying the challenges, risks, and mitigation strategies associated with involving an industrial company as product owner in a project course. Those elements have been taken into consideration when planning the next instance of the course& When addressing a specific question in the model, say observed problems from the perspective of students, it is often difficult to separate between what we teachers think and what students have actually reported. Ideally, the template should have been filled by different course stakeholders: teachers, teaching assistants, students, and external company& Involving an external company might widen the gap between the expected course learning objectives and the actual learning outcomes experienced by students & Apply the model to communicate the experiences of the first instance of the course to the different stakeholders highlighting both the success stories and observed problems. Formulate the experiences around the different elements of the model.\tabularnewline

\midrule
PA243 & Industrial contacts for master thesis projects & N/A & Model v3 allowed for more creativity in the analysis\newline Version 6 of the model allowed for a detailed analysis of the different stakeholders & The result from model v3 was harder to compare to results from other courses\newline Model v6 took more time to fill out & The model exposed why certain changes to the course worked and others did not, and for whom & It is worth knowing the roles of the external stakeholders to better assess changes to a course\tabularnewline
\midrule
TDA593/DIT945 & Industrial guest lecturers & (to apply the model) 1-2 hours & Easy to apply\newline Helped to understand in depth stakeholder aims. This uncovered potential sources of conflict and/or friction between the stakeholders and the course responsibles or students. & Differences between some questions were not clear. Some questions felt repetitive. & Misalignment between student background and abstraction level of guest lectures, lack of alignment of the guest lecture content with the remainder of the course & (Planned) Follow-up lectures to explain/put into context the guest lectures. Discussion sessions with the teachers in the end of each guest lecture. More preparation of guest lecturers before their lecture. \tabularnewline

\bottomrule
\end{tabular}}
\label{tab:source-type-provenance-1}
\end{table}


\end{landscape}}
